NAS-DIP: Learning Deep Image Prior with Neural Architecture Search

Recent work has shown that the structure of deep convolutional neural networks can be used as a structured image prior for solving various inverse image restoration tasks. Instead of using hand-designed architectures, we propose to search for neural architectures that capture stronger image priors. Building upon a generic U-Net architecture, our core contribution lies in designing new search spaces for (1) an upsampling cell and (2) a pattern of cross-scale residual connections. We search for an improved network by leveraging an existing neural architecture search algorithm (using reinforcement learning with a recurrent neural network controller). We validate the effectiveness of our method via a wide variety of applications, including image restoration, dehazing, image-to-image translation, and matrix factorization. Extensive experimental results show that our algorithm performs favorably against state-of-the-art learning-free approaches and reaches competitive performance with existing learning-based methods in some cases.

==> figure/fig_inpainting.tex <==
\begin{figure}[!t]
  \begin{center}
  \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-input-box.png}} \hfill
  \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-GT-box.png}} \hfill
  \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-DIP-box.png}} \hfill
  \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-Ours-box.png}} \\
  \mpage{0.23}{\includegraphics[width=0.47\linewidth]{image/inpainting-crop/barbara-input-1.png} \hfill \includegraphics[width=0.47\linewidth]{image/inpainting-crop/barbara-input-2.png}} \hfill
  \mpage{0.23}{\includegraphics[width=0.47\linewidth]{image/inpainting-crop/barbara-GT-1.png} \hfill \includegraphics[width=0.47\linewidth]{image/inpainting-crop/barbara-GT-2.png}} \hfill
  \mpage{0.23}{\includegraphics[width=0.47\linewidth]{image/inpainting-crop/barbara-DIP-1.png} \hfill \includegraphics[width=0.47\linewidth]{image/inpainting-crop/barbara-DIP-2.png}} \hfill
  \mpage{0.23}{\includegraphics[width=0.47\linewidth]{image/inpainting-crop/barbara-Ours-1.png} \hfill \includegraphics[width=0.47\linewidth]{image/inpainting-crop/barbara-Ours-2.png}} \\
  \vspace{1.0mm}
  \mpage{0.23}{Corrupted image} \hfill
  \mpage{0.23}{Ground truth} \hfill
  \mpage{0.23}{DIP~\cite{DIP-CVPR-2018}} \hfill
  \mpage{0.23}{Ours} \\
  \vspace{\figcapmargin}
  \caption{
  \textbf{Qualitative results of image inpainting.} 
  We present visual comparisons with DIP~\cite{DIP-CVPR-2018} on the dataset provided by \cite{Heide-CVPR-2015}.
  }
  \label{fig:inpainting}
  \end{center}
  \vspace{\figmargin}
\end{figure}

% \begin{figure}[t]
%   \begin{center}
%   %
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-input-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-GT-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-DIP-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-Ours-box.png}} \\
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-input-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-input-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-GT-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-GT-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-DIP-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-DIP-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-Ours-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/barbara-Ours-2.png}}} \\
%   %
%   \vspace{3.0mm}
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/boat-input-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/boat-GT-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/boat-DIP-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/boat-Ours-box.png}} \\
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/boat-input-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/boat-input-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/boat-GT-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/boat-GT-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/boat-DIP-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/boat-DIP-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/boat-Ours-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/boat-Ours-2.png}}} \\
%   %
%   \vspace{3.0mm}
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/Cameraman256-input-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/Cameraman256-GT-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/Cameraman256-DIP-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/Cameraman256-Ours-box.png}} \\
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Cameraman256-input-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Cameraman256-input-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Cameraman256-GT-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Cameraman256-GT-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Cameraman256-DIP-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Cameraman256-DIP-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Cameraman256-Ours-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Cameraman256-Ours-2.png}}} \\
%   %
%   \vspace{3.0mm}
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/couple-input-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/couple-GT-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/couple-DIP-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/couple-Ours-box.png}} \\
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/couple-input-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/couple-input-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/couple-GT-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/couple-GT-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/couple-DIP-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/couple-DIP-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/couple-Ours-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/couple-Ours-2.png}}} \\
%   %
%   \mpage{0.23}{Corrupted image} \hfill
%   \mpage{0.23}{Ground truth} \hfill
%   \mpage{0.23}{DIP~\cite{DIP-CVPR-2018}} \hfill
%   \mpage{0.23}{Ours} \\
%   %
%   \vspace{-2.0mm}
%   \captionof{figure}{\textbf{Qualitative results of image inpainting.} We present visual comparisons with DIP~\cite{DIP-CVPR-2018} on the dataset provided by \cite{Heide-CVPR-2015}.}
%   \label{fig:inpainting}
%   \end{center}
% \end{figure}

% \begin{figure}[t]
%   \begin{center}
%   %
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/fingerprint-input-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/fingerprint-GT-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/fingerprint-DIP-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/fingerprint-Ours-box.png}} \\
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/fingerprint-input-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/fingerprint-input-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/fingerprint-GT-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/fingerprint-GT-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/fingerprint-DIP-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/fingerprint-DIP-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/fingerprint-Ours-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/fingerprint-Ours-2.png}}} \\
%   %
%   \vspace{3.0mm}
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/hill-input-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/hill-GT-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/hill-DIP-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/hill-Ours-box.png}} \\
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/hill-input-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/hill-input-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/hill-GT-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/hill-GT-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/hill-DIP-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/hill-DIP-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/hill-Ours-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/hill-Ours-2.png}}} \\
%   %
%   \vspace{3.0mm}
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/house-input-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/house-GT-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/house-DIP-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/house-Ours-box.png}} \\
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/house-input-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/house-input-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/house-GT-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/house-GT-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/house-DIP-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/house-DIP-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/house-Ours-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/house-Ours-2.png}}} \\
%   %
%   \vspace{3.0mm}
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/Lena512-input-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/Lena512-GT-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/Lena512-DIP-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/Lena512-Ours-box.png}} \\
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Lena512-input-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Lena512-input-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Lena512-GT-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Lena512-GT-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Lena512-DIP-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Lena512-DIP-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Lena512-Ours-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/Lena512-Ours-2.png}}} \\
%   %
%   \mpage{0.23}{Corrupted image} \hfill
%   \mpage{0.23}{Ground truth} \hfill
%   \mpage{0.23}{DIP~\cite{DIP-CVPR-2018}} \hfill
%   \mpage{0.23}{Ours} \\
%   %
%   \vspace{-2.0mm}
%   \captionof{figure}{\textbf{Qualitative results of image inpainting.} We present visual comparisons with DIP~\cite{DIP-CVPR-2018} on the dataset provided by \cite{Heide-CVPR-2015}.}
%   \label{fig:inpainting-2}
%   \end{center}
% \end{figure}

% \begin{figure}[t]
%   \begin{center}
%   %
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/man-input-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/man-GT-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/man-DIP-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/man-Ours-box.png}} \\
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/man-input-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/man-input-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/man-GT-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/man-GT-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/man-DIP-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/man-DIP-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/man-Ours-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/man-Ours-2.png}}} \\
%   %
%   \vspace{3.0mm}
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/montage-input-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/montage-GT-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/montage-DIP-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/montage-Ours-box.png}} \\
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/montage-input-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/montage-input-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/montage-GT-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/montage-GT-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/montage-DIP-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/montage-DIP-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/montage-Ours-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/montage-Ours-2.png}}} \\
%   %
%   \vspace{3.0mm}
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/peppers256-input-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/peppers256-GT-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/peppers256-DIP-box.png}} \hfill
%   \mpage{0.23}{\includegraphics[width=\linewidth]{image/inpainting-crop/peppers256-Ours-box.png}} \\
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/peppers256-input-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/peppers256-input-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/peppers256-GT-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/peppers256-GT-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/peppers256-DIP-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/peppers256-DIP-2.png}}} \hfill
%   \mpage{0.23}{\mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/peppers256-Ours-1.png}} \hfill \mpage{0.45}{\includegraphics[width=\linewidth]{image/inpainting-crop/peppers256-Ours-2.png}}} \\
%   %
%   \mpage{0.23}{Corrupted image} \hfill
%   \mpage{0.23}{Ground truth} \hfill
%   \mpage{0.23}{DIP~\cite{DIP-CVPR-2018}} \hfill
%   \mpage{0.23}{Ours} \\
%   %
%   \captionof{figure}{\textbf{Qualitative results of image inpainting.} We present visual comparisons with DIP~\cite{DIP-CVPR-2018} on the dataset provided by \cite{Heide-CVPR-2015}.}
%   \label{fig:inpainting-3}
%   \end{center}
% \end{figure}
